Factor Graph Accelerator for LiDAR-Inertial Odometry

Factor graph is a graph representing the factorization of a probability distribution function, and has been utilized in many autonomous machine computing tasks, such as localization, tracking, planning and control etc. We are developing an architecture with the goal of using factor graph as a common abstraction for most, if not, all autonomous machine computing tasks. If successful, the architecture would provide a very simple interface of mapping autonomous machine functions to the underlying compute hardware. As a first step of such an attempt, this paper presents our most recent work of developing a factor graph accelerator for LiDAR-Inertial Odometry (LIO), an essential task in many autonomous machines, such as autonomous vehicles and mobile robots. By modeling LIO as a factor graph, the proposed accelerator not only supports multi-sensor fusion such as LiDAR, inertial measurement unit (IMU), GPS, etc., but solves the global optimization problem of robot navigation in batch or incremental modes. Our evaluation demonstrates that the proposed design significantly improves the real-time performance and energy efficiency of autonomous machine navigation systems. The initial success suggests the potential of generalizing the factor graph architecture as a common abstraction for autonomous machine computing, including tracking, planning, and control etc.

==> traits-bk.tex <==
\section{Traits of Factor Graph Computing}
\label{sec:traits}

% \fixme{always have a space before ``(''}   ----done.

We first introduce the general MAP inference formulation for factor graphs, including both batch optimization and incremental smoothing problems (\Sect{sec:traits:map}). Then we propose a dedicated algorithm for solving the LIO factor graph (\Sect{sec:traits:sol}) and analyze how its special graph structure can be used to speed up the inference performance (\Sect{sec:traits:para}).

\subsection{MAP Inference for Factor Graph}
\label{sec:traits:map}
% We first introduce how to solve a factor graph in batch given an unknown factor graph. Then we present how to solve incrementally based on a factor graph that has already been solved and new data.
\fixme{1. what a general factor graph look like; 2. the method to turn the factor graph into a MAP problem; 3. incremental smoothing on factor graph; Refer to our bundle adjustment paper.}

Factor graph is a bipartite graph of which structure represents a factorization of a global function. It has two types of nodes. One is the variable node $X$, which represents the unknown states; and the other is the factor node $\phi$, which denotes the constraints between the variables connected to it. Thus, a factor graph factorizes a global function $\Phi(X)$ into a series of products of factors that are simply functions of the local variables connected to it, as
\begin{equation}
    \centering
    \Phi(X)=\prod_i\phi_i(X_i)
    \label{equ:factorize}
\end{equation}

In many AMC problems, we are typically interested in the unknown states $X$, such as poses (position and orientation), given the measurements $Z$. Factor graph can model these estimation problems elegantly and concisely, using variable nodes represent $X$ and factor nodes denote the constraints formed by $Z$. We then seek to derive a set of states that maximize the value of the global function corresponding to factor graph. That is, MAP inference is performed on factor graph:
\begin{equation}
    X^{MAP}=\mathop{\arg\max}\limits_X\Phi(X)=\mathop{\arg\max}\limits_X\prod_i\phi_i(X_i)
    \label{equ:mapmax}
\end{equation}

Assuming that all factors are of the form as \Equ{equ:exp}, which include both simple Gaussian priors and likelihood factors derived from measurements corrupted by zero-mean, normally distributed noise, where $z_i$ is the $i$-th measurement or ground truth, $h_i(\cdot)$ is a measurement function that maps the state $X_i$ to be estimated to its sensor's measurement space, $\Sigma_i$ is the covariance matrix of the $i$-th measurement and $\Vert\cdot\Vert^2_{\Sigma}$ is the Mahalanobis norm that quantifies the error. Taking the negative log of \Equ{equ:mapmax} allows us to instead minimize a sum of nonlinear least-squares as \Equ{equ:mapmin}.
\begin{equation}
    \phi_i(X_i)\propto\exp{\Vert h_i(X_i)-z_i \Vert^2_{\Sigma_i}}
    \label{equ:exp}
\end{equation}
\begin{equation}
    X^{MAP}=\mathop{\arg\min}\limits_X\sum_i\Vert h_i(X_i)-z_i \Vert^2_{\Sigma_i}
    \label{equ:mapmin}
\end{equation}

Nonlinear least-squares problems cannot be solved directly, but require an iterative solution starting from an initial estimate. Both the Gaussian-Newton method and the Levenberg-Marquardt algorithm share the following basic structure: They start from an initial $X^0$. In each iteration, an increment $\Delta$ is computed and applied to obtain the next estimate $X^*=X^0+\Delta$. This process ends when certain convergence criteria are reached, such as the change $\Delta$ falling below a small threshold.

Substituting the Taylor expansion of $h_i(X_i)$ into the nonlinear least-squares expression (\Equ{equ:mapmin}) we obtain a linear least-squares problem in the state increment $\Delta$:
\begin{equation}
    \Delta^*=\mathop{\arg\min}\limits_\Delta\sum_i\Vert H_i\Delta_i-(z_i-h_i(X_i^0)) \Vert^2_{\Sigma_i}
    \label{equ:mapdelta}
\end{equation}
where the measurement Jacobian $H_i$ is defined as the partial derivative of $h_i(\cdot)$ at a given linearization point $X^0$. By a simple change of variables the covariance matrices $\Sigma_i$ can be dropped ~\cite{dellaert2017factor}. We finally obtain the following standard least-squares problem,
\begin{align}
    \Delta^*&=\mathop{\arg\min}\limits_\Delta\sum_i\Vert A_{bi}\Delta_i-\epsilon_{bi}\Vert^2_2 \nonumber\\
    &=\mathop{\arg\min}\limits_\Delta\Vert A_{b}\Delta-\epsilon_{b}\Vert^2_2
    \label{equ:mapmatrix}
\end{align}
where $A_b$ and $\epsilon_b$ are obtained by collecting all Jacobian matrices $A_{bi}$ and residuals $\epsilon_{bi}$ into one large matrix $A_b$ and right-hand-side (RHS) vector $\epsilon_b$, respectively. In fact, the factor nodes in factor graph store the entries in $\epsilon_b$ and $A_b$, and the structure of factor graph is equivalent to the sparse pattern of $A_b$. In more detail, each block row in $A_b$ corresponds to a factor node; each block column in $A_b$ corresponds to a variable node.

Given a factor graph, there exits a general algorithm, namely Variable Elimination (VE)~\cite{dellaert2017factor}, which is capable of computing the $\Delta^*$ in \Equ{equ:mapmatrix}. VE factorizes the global function $\Phi(\Delta)$ corresponding to the factor graph into a Bayes net probability density as,
\begin{equation}
    \counterwithin{equation}{section}
    % \frac{1}{Z}\phi(X) = p(x_1|S_1)p(x_2|S_2)\cdots p(x_n) = \prod\limits_j p(x_j|S_j)
    \Phi(\Delta) = p(\delta x_1|S_1)p(\delta x_2|S_2)\cdots p(\delta x_n) = \prod\limits_j p(\delta x_j|S_j)
    \label{equ:ve}
\end{equation}
where $S_j$ denotes the separator associated with the increment $\delta x_j$; the separators are a set of variables on which $\delta x_j$ is conditioned after being eliminated (\fixme{what does "being eliminated" mean}), which means the variables contained in $S_j$ must be known while solving for $\delta x_j$. (\fixme{cann't see how a factor graph comes to the above formula})

From the perspective of linear algebra, as shown in \Equ{equ:qr}, the QR decomposition of $A_b$ is equivalent to the variable elimination of factor graph. The obtained upper triangular matrix $R$, also called the square root information matrix, corresponds to the Bayes net. In other words, the $j$-th block row in $R$ corresponds to $p(\delta x_j|S_j)$ in the Bayes net. Then $\Delta$ can be solved by back substitution on the Bayes net. 
\begin{align}
    \mathop{\arg\min}\limits_\Delta\Vert A_b\Delta-\epsilon_b \Vert^2_2&=\mathop{\arg\min}\limits_\Delta\Vert Q^TA_b\Delta-Q^T\epsilon_b \Vert^2_2 \nonumber\\
                                                                       &=\mathop{\arg\min}\limits_\Delta\Vert R\Delta-d \Vert^2_2
    \label{equ:qr}
\end{align}

% \begin{algorithm}[tb]
%     \counterwithin{algorithm}{section}
%     \caption{The Variable Elimination Algorithm}
%     \label{alg:VE}
%     \begin{algorithmic}[1]
%         \Function{E{\footnotesize LIMINATE}}{$\Phi_{1:n}$}
%         \For{$i=1$ to $n$}
%         \State $p(x_i|S_i)$,$\Phi_{i+1:n}\gets$ E{\footnotesize LIMINATE}O{\footnotesize NE}($\Phi_{i:n}$,$x_i$)
%         \EndFor
%         \State\Return $p(x_1|S_1)p(x_2|S_2)\cdots p(x_n)$
%         \EndFunction
%     \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[tb]
%     \caption{Eliminate $x_j$ From Factor Graph $\Phi_{j:n}$}
%     \label{alg:VEONE}
%     \begin{algorithmic}[1]
%         \Function{E{\footnotesize LIMINATE}O{\footnotesize NE}}{$\Phi_{j:n}$,$x_j$}
%         \State Remove all factors $\phi_i(x_i)$ that are adjacent to $x_j$
%         \State $S_j\gets$ all variables involved excluding $x_j$
%         \State $\psi(x_j, S_j) \gets \prod\nolimits_i\phi_i(x_i)$
%         \State $p(x_j|S_j)\tau(S_j) \gets \psi(x_j, S_j)$
%         \State Add the new factor $\tau(S_j)$ back into the graph
%         \State\Return $p(x_j|S_j)$,$\Phi_{j+1:n}$
%         \EndFunction
%     \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[tb]
    \counterwithin{algorithm}{section}
    \caption{The Variable Elimination Algorithm}
    \label{alg:VE}
    \begin{algorithmic}[1]
        \Function{VE}{$\Phi_{1:n}$}
        \For{$i=1$ to $n$}
        \State Remove all factors $\phi_i(\cdot)$ that are adjacent to $x_i$
        \State $S_i\gets$ all variables involved in $\phi_i(\cdot)$ excluding $x_i$
        \State $\psi(x_i, S_i) \gets \prod\nolimits_i\phi_i(x_i)$
        \State $p(x_i|S_i)\tau(S_i) \gets \psi(x_i, S_i)$
        \State Add the new factor $\tau(S_i)$ back into the graph
        \EndFor
        \State\Return $p(x_1|S_1)p(x_2|S_2)\cdots p(x_n)$
        \EndFunction
    \end{algorithmic}
\end{algorithm}

\Alg{alg:VE} shows the process of variable elimination on a factor graph corresponding to \Equ{equ:ve} and \Equ{equ:qr}. Starting with an initial factor graph $\Phi(x_{1:n})$, each elimination of a variable $x_i$ yields a conditional probability $p(x_i|S_i)$ as well as a factor graph $\Phi(x_{i+1:n})$ over the remaining variables. A Bayes net is returned after all variables have been eliminated.
% The input is an initial or partially eliminated factor graph $\Phi(x_{j:n})$. Factors $\phi_j(x_j)$ adjacent to $x_j$ are first removed. Then the product $\psi(x_j, S_j)$  of these factors is factorized into a conditional probability $p(x_j|S_j)$ and a new factor $\tau(S_j)$. Finally insert $\tau(S_j)$ into $\Phi(x_{j+1:n})$ and return $p(x_j|S_j)$. When eliminating the last variable $x_n$, the separator $S_n$ is empty so that only the prior probability $p(x_n)$ is obtained, which also means that the MAP solution of $x_n$ can be directly solved without depend on any variables.

Assuming that the data is all available in advance, we can solve the batch optimization efficiently using only \Alg{alg:VE}. However, data is obtained as a temporal sequence in many inference problems for autonomous machines. This leads to an unavoidable problem that, when new data arrives, whether to use the previous results to optimize incrementally or to perform a  batch optimization every time. In fact, efficient incremental smoothing can reuse the results of previous steps~\cite{kaess2012isam2}, which can avoid the unaffordable time overhead caused by iterative batch optimization. The process of incremental smoothing is an update to a new data structure, the Bayes tree, that is a directed tree of which nodes consist of the cliques in the Bayes net obtained by eliminating a factor graph. When new measurements arrive, only those affected nodes need to be removed and reconstructed to a factor graph where new factors are inserted. Then eliminate this factor graph with \Alg{alg:VE} and transform the resulting Bayes net into a Bayes tree. Finally, the unaffected subtrees are inserted into it. The pseudocode of incremental smoothing is shown in \Alg{alg:UPD}. We will illustrate the above algorithms in detail with some toy examples and propose the dedicated algorithm for solving LIO factor graph in \Sect{sec:traits:sol}.

% In fact, efficient incremental smoothing can reuse the results of previous steps~\cite{kaess2012isam2}, which can avoid the unaffordable time overhead caused by iterative batch optimization. The process of incremental smoothing is an update to a new data structure, the Bayes tree, that is a directed tree of which nodes consist of the cliques in the Bayes net obtained by eliminating a factor graph. The pseudocode of incremental smoothing is shown in \Alg{alg:UPD}. We will illustrate the above algorithms in detail with some toy examples and propose the dedicated algorithm for solving LIO factor graph in \Sect{sec:traits:sol}.

\begin{algorithm}[tb]
    \caption{Update The Bayes Tree}
    \label{alg:UPD}
    \begin{algorithmic}[1]
        \Function{U{\footnotesize PDATE}B{\footnotesize AYES}T{\footnotesize REE}}{Bayes tree $\mathcal T$, new factor $f(\mathcal J)$}
        \State For each affected variable in $\mathcal J$:
        \State Remove corresponding clique and all parents up to root
        \State Store orphaned sub-trees $\mathcal T_{orph}$ of removed cliques
        \State Convert removed cliques to factor graph and add $f(\mathcal J)$
        \State Eliminate the factor graph into a Bayes net
        \State Create a new Bayes tree $\mathcal T^{'}$  from this new Bayes net
        \State Insert the orphans $\mathcal T_{orph}$ back into $\mathcal T^{'}$
        \State \Return the updated Bayes Tree $\mathcal T^{'}$
        \EndFunction
    \end{algorithmic}
\end{algorithm}

\subsection{Solving for LIO Factor Graph}
\label{sec:traits:sol}
\fixme{LIO problem formulation: problem description; factor graph representation; algorithm operations/architecture to solve the MAP of factor graph. Refer to our bundle adjustment paper.}

% The factor graph corresponding to the LiDAR-inertial odometry has a chain-like structure. If it is capable of loop closure detection, only a few loop closure factors are added to the chain factor graph, which destroys the good property of pure chain structure, as shown in \Fig{fig:lio}. However, it still results in a factor graph that is rich in regularity when solving for the MAP solution. The approximate chain-like property avoids the necessity of traversing the factor graph before solving it, saving time and space overhead.
LIO uses GPS, IMU and LiDAR as the main sensors. GPS measurements generate constraints on the position of each keyframe; IMU measurements yield constraints on the poses, velocities, acceleration and gyroscope biases of two adjacent keyframes; and LiDAR measurements produce constraints on the poses of two adjacent keyframes. Thus, the LIO factor graph has a chain-like structure, as shown in \Fig{fig:liofg}. The factor nodes are composed of three sensors, and the variable nodes include the pose, velocity and biases of each keyframe. It results in a factor graph that is rich in regularity when solving for the MAP solution. The chain-like property avoids the necessity of traversing the factor graph before solving it, saving time and space overhead.

\begin{figure}[t]
    \counterwithin{figure}{section}
    \centering
    \includegraphics[width=0.9\columnwidth]{liofg}
    \caption{Factor graph of tightly coupled LiDAR-inertial odometry. The hollow nodes represent the pose, velocity and bias variables. The solid nodes denote the different factors.} %Circular nodes are variable nodes, including pose, velocity and bias. Square nodes are factor nodes, including gps factor, LiDAR/loop closure factor and imu factor.}
    \label{fig:liofg}
\end{figure}


\begin{figure*}[htbp]
    \centering
    \subfigure[]{
        \label{fig:sve1}
        \includegraphics[width=0.63\columnwidth]{sve_new1}}
    % \hspace{-0.5in}
    \subfigure[]{
        \label{fig:sve2}
        \includegraphics[width=0.63\columnwidth]{sve_new2}}
    % \hspace{-0.5in}
    \subfigure[]{
        \label{fig:sve3}
        \includegraphics[width=0.63\columnwidth]{sve_new3}}
    \setlength{\abovecaptionskip}{0.cm}
    \caption{Factor graph and corresponding matrix obtained using serial elimination. (a) Toy example of LIO factor graph with four variables and its corresponding Jacobian matrix  $A_b$ in serial elimination order. (b) Factor graph and the corresponding matrix after eliminating $x_1$. (c) The Bayes net obtained using serial elimination and the corresponding square root information matrix $R$.}
    \label{fig:SVE}
\end{figure*}

% \begin{algorithm}[b]
%     \caption{Elimination $x_j$ From LIO Factor Graph}
%     \label{alg:lio_eli_one}
%     \begin{algorithmic}[1]
%         \Function{E{\footnotesize LIMINATE}O{\footnotesize NE}}{$g_j$, $b_j$, $\tau_j$}
%         \State Construct $\overline{A_j}$ with $g_j$, $b_j$ and $\tau_j$
%         \State Perform partial QR decomposition on $\overline{A_j}$
%         \State\Return $p(x_j|x_{j+1})$, $\tau_{j+1}$
%         \EndFunction
%     \end{algorithmic}    
%     % \vspace{-5pt}
% \end{algorithm}
\begin{algorithm}[ht]
    \counterwithin{algorithm}{section}
    \caption{The VE Algorithm on LIO Factor Graph}
    \label{alg:VELIO}
    \begin{algorithmic}[1]
        \Function{VE\_LIO}{$\Phi_{1:n}$}
        \For{$i=1$ to $n$}
        \State Construct $\overline{A_i}$ with $g_i$, $b_i$ and $\tau_i$
        \State  $p(x_i|x_{i+1})$, $\tau_{i+1}$ $\gets$ partial QR decomposition on $\overline{A_i}$
        \EndFor
        \State\Return $p(x_1|x_2)p(x_2|x_3)\cdots p(x_n)$
        \EndFunction
    \end{algorithmic}
\end{algorithm}
% \begin{algorithm}[b]
%     \caption{Incremental Inference On LIO Factor Graph}    
%     \label{alg:lio_incre}
%     \begin{algorithmic}[1]
%         \Function{I{\footnotesize NCREMENTAL}I{\footnotesize NFERENCE}}{$g_{j+1}$, $b_{j}$}
%         \State Reconstruct the factor graph $\Phi_{j-1:j+1}$ of $x_{j-1}, x_{j}$ and $x_{j+1}$
%         \For{$i=j-1$ to $j+1$}
%         \State $p(x_i|x_{i+1})$, $\tau_i$ $\gets$ E{\footnotesize LIMINATE}O{\footnotesize NE}($g_i$, $b_i$, $\tau_{i-1}$)
%         \EndFor
%         \State \Return $p(x_{j-1}|x_j)p(x_{j}|x_{j+1})p(x_{j+1})$
%         \EndFunction
%     \end{algorithmic}
%     % \vspace{-5pt}
% \end{algorithm}
\begin{algorithm}[ht]
    \caption{Incremental Inference On LIO Factor Graph}    
    \label{alg:lio_incre}
    \begin{algorithmic}[1]
        \Function{I{\footnotesize NCREMENTAL}I{\footnotesize NFERENCE}}{$g_{j+1}$, $b_{j}$}
        \State Reconstruct the factor graph $\Phi_{j-1:j+1}$ of $x_{j-1}, x_{j}$ and $x_{j+1}$
        \State VE\_LIO($\Phi_{j-1:j+1}$)
        \State \Return $p(x_{j-1}|x_j)p(x_{j}|x_{j+1})p(x_{j+1})$
        \EndFunction
    \end{algorithmic}
    % \vspace{-5pt}
\end{algorithm}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{update_new}
    \caption{Incremental update using Bayes tree. New measurements only affect the root clique, only this part is recalculated (shown in red).}
    \label{fig:updateBT}
    \vspace{-8pt}
\end{figure}

% The case of no loop closure detection is discussed first. 
\Fig{fig:sve1} shows the LIO factor graph for a toy example and its corresponding Jacobian matrix $A_b$(\fixme{how comes the Jacobian}), where the velocity and biases variables as well as the IMU factors are omitted for the sake of brevity and clarity. If the forward elimination order of $x_1\to x_2\to x_3\to x_4$ is selected, the adjacent factors $g_1(x_1)$ and $b_1(x_1,x_2)$ need to be removed when eliminating $x_1$, then multiplied into the product $\psi(x_1,x_2)$ and factorized into a conditional probability $p(x_1|x_2)$ and a new factor $\tau(x_2)$, that is
% \begin{equation}
\begin{align}
    \psi(x_1,x_2) & \gets g_1(x_1)b_1(x_1,x_2) \label{prod} \\
    \psi(x_1,x_2) & \to p(x_1|x_2)\tau(x_2)   \label{deco}
\end{align}
% \end{equation}

From the perspective of the matrix, \Equ{prod} corresponds to the process of constructing a matrix $\overline{A}$. In contrast, \Equ{deco} represents the process of decomposing $\overline{A}$. When eliminating $x_1$, $\overline{A_1} = \begin{bmatrix} A_{11} & \\ A_{51} & A_{52} \end{bmatrix}$. Then perform partial $QR$ decomposition on $\overline{A_1} = Q_1\begin{bmatrix} R_{1} & T_{12}\\   & \tau_{52} \end{bmatrix}$, where $R_{1}$ is an upper triangular matrix, as shown in \Fig{fig:sve2}. However, factors adjacent to $x_j$ to be eliminated are fixed due to the chain-like nature of LIO factor graph, i.e., only a GPS factor $g_j(x_j)$, a LiDAR factor $b_j(x_j,x_{j+1})$, and a new factor $\tau(x_j)$ obtained by the last elimination are involved. Besides, the separator $S_j$ contains only $x_{j+1}$. Therefore, the matrix $\overline{A_j}$ can be directly constructed without traversing the factor graph. The obtained Bayes net is shown in \Fig{fig:sve3} after all variables are eliminated. When solving the MAP solution in back substitution, the reverse order of the elimination should be followed, i.e., $x_4\to x_3\to x_2\to x_1$ should be solved in turn. \Alg{alg:VELIO} shows pseudocode for eliminating a LIO factor graph.

When solving LIO factor graph incrementally, a chain Bayes tree is used to maintain the square root information matrix at each moment. Following \Alg{alg:UPD}, only the root clique in the Bayes tree is removed and a factor graph of the two nearest variable nodes is reconstructed. Then insert the new factors into the graph. That is, whenever the chained Bayes tree is updated, only a factor graph containing three variables needs to be eliminated, as shown in \Fig{fig:updateBT}. \Alg{alg:lio_incre} shows pseudocode for incremental inference on LIO factor graph.



\begin{figure}[t]
    \centering
    \subfigure[]{
        \label{fig:pve2}
        \includegraphics[width=0.48\columnwidth]{pve_new1}}
    % \hspace{0.5in}
    \subfigure[]{
        \label{fig:pve3}
        \includegraphics[width=0.48\columnwidth]{pve_new2}}
    \setlength{\abovecaptionskip}{0.cm}
    \caption{Factor graph and corresponding matrix obtained using parallel elimination. (a) Factor graph and the corresponding matrix after eliminating $x_1$ and $x_4$ simultaneously. (b) The Bayes net obtained using parallel elimination and the corresponding square root information matrix $R$. }
    \vspace{-0.1in}
    \label{fig:PVE}
\end{figure}

\begin{algorithm}[tb]
    \counterwithin{algorithm}{section}
    \caption{The Parallel VE Algorithm on LIO Factor Graph}
    \label{alg:PVELIO}
    \begin{algorithmic}[1]
        \Function{PVE\_LIO}{$\Phi_{1:n}$}
        \For{$i=1$ to $\frac{n}{2}$}
        \If{no conflicting factor between $x_i$ and $x_{n-i}$}
        \State Construct $\overline{A_i}$ and $\overline{A}_{n-i}$
        \State  $p(x_i|x_{i+1})$, $p(x_{n-i}|x_{n-i-1})$ $\stackrel{pQR}{\longleftarrow}$ $\overline{A_i}$, $\overline{A}_{n-i}$
        \Else
        \State Construct $\overline{A_i}$
        \State  $p(x_i|x_{i+1})$ $\stackrel{pQR}{\longleftarrow}$  $\overline{A_i}$
        \EndIf
        \EndFor
        \State\Return $p(x_1|x_2)\cdots p(x_\frac{n}{2})\cdots p(x_n|x_{n-1})$
        \EndFunction
    \end{algorithmic}
\end{algorithm}


\subsection{Parallel Computation of LIO Factor Graph}
\label{sec:traits:para}
\fixme{evidence of parallel computing for LIO factor graph: explain the idea; prove the idea; show the algorithm of parallel algorithm.}

We now explore the parallel computation of elimination and back substitution by considering the symmetric properties of LIO factor graph to accelerate the inference. 

When eliminating $x_1$, there is no conflict between its adjacent factors and those of $x_4$. Therefore, the elimination of $x_1$ and $x_4$ is considered simultaneously. The factors involved are exactly the same so that the dimension of the matrices $\overline{A_1}$ and $\overline{A_4}$ corresponding to the two product factors $\psi(x_1,x_2)$ and $\psi(x_3, x_4)$, respectively, are exactly identical. The new factors $\tau(x_2)$ and $\tau(x_3)$ are obtained after the parallel elimination is completed, as shown in \Fig{fig:pve2}. Parallel elimination could continue if the chain was longer, but not in this case because $x_2$ and $x_3$ have common factor $b_2(x_2,x_3)$ here. Moreover, for the same length of the chain factor graph, the maximum dimension of the matrix to be decomposed for parallel elimination is smaller than that for serial elimination.  \Alg{alg:PVELIO} shows pseudocode for parallel VE algorithm for LIO factor graph. Parallel elimination also results in a different Bayes net as shown in \Fig{fig:pve3}, in which case the root of the Bayes net is in the middle and the directed edges point to the variables on both sides. This means that the root variable can be solved first, after which the children variables on both sides can be solved in parallel in turn.

It is interesting that the two elimination patterns get the same filling-in with different elimination orders --- they are all three in this toy example. However, the competitiveness of parallel elimination is reflected in: (a) parallelization of the matrix decomposition (b) dimension reduction of the matrix to be decomposed and (c) parallelization of the back substitution.

Parallel elimination can also be employed for incremental smoothing of LIO factor graph. Therefore, it is also accelerated by parallel elimination.

% If the loop closure factor is introduced, the factor graph becomes more complicated due to the loss of the pure chain property. Fortunately, the regularities still exist in the process of elimination. If there is a loop closure factor $c(x_i, x_j)$ between $x_i$ and $x_j$, the factors involved in the elimination of $x_i$ contain the factor $c(x_i, x_j)$, in addition to the GPS factor $g(x_i)$, the LiDAR factor $b(x_i, x_{i+1})$ and the new factor $\tau_i(x_i)$ in the no-loop case. The variables involved are newly added $x_j$ on the basis $x_i$ and $x_{i+1}$ of the original. This effect persists until elimination $x_{j-1}$. If there is a new loop closure factor during this period, this process continues iteratively. When a loop closure factor is encountered in incremental mode, it is necessary to reconstruct the factor graph of all the variables between the loop, and then solve this cyclic factor graph by elimination. Similarly, parallel elimination can be started from two variables with no common factors, as shown in \Fig{}. The pseudocode for solving the LIO factor graph in batch and incrementally is given in \Alg{} and \Alg{}, respectively.

% \begin{algorithm}[tb]
%     \caption{Elimination Of $x_j$ In The LIO Factor Graph}
%     \label{alg:lio_eli_one}
%     \begin{algorithmic}[1]
%         \Function{E{\footnotesize LIMINATE}O{\footnotesize NE}}{$g_j$, $b_j$, $\tau(S_{j-1})$, $C$, $x_j$, $S_{j-1}$}
%         \State Remove $x_{j}$ from $S_{j-1}$
%         \State $S_j \gets S_{j-1}$
%         \State Add $x_{j+1}$ to $S_{j}$

%         \State Construct $\overline{A_j}$ with $g_j$, $b_j$ and $\tau(S_{j-1})$
%         \If{$c_{jk} \in C$}
%         \State Add $x_k$ to $S_j$
%         \State Add $c_{jk}$ to $\overline{A_j}$
%         \EndIf
%         \State Perform partial QR decomposition on $\overline{A_j}$
%         \State\Return $p(x_j|S_j)$, $\tau(S_j)$
%         \EndFunction
%     \end{algorithmic}    
% \end{algorithm}


% \begin{algorithm}
%     \caption{Incremental Inference On The LIO Factor Graph}    
%     \label{alg:lio_incre}
%     \begin{algorithmic}[1]
%         \Function{I{\footnotesize NCREMENTAL}I{\footnotesize NFERENCE}}{$g_{j}$, $b_{j-1}$, $x_{j}$, $C_r(X)$, $c_{ij}$}
%         \If{$c_{ij}$}
%         \State reconstruct a cyclic $\Phi_{1:n}$ between $x_i$ and $x_j$
%         \Else 
%         \State reconstruct a chain $\Phi_{1:n}$ with $x_{j}$ and $C_r(X)$        
%         \EndIf
%         \For{$i=1$ to $n$}
%         \State 
%         \EndFor
%         \EndFunction
%     \end{algorithmic}
% \end{algorithm}
